Take More Positives: An Empirical Study of Contrastive Learing in Unsupervised Person Re-Identification

Unsupervised person re-identification (re-ID) aims at closing the performance gap to supervised methods. These methods build reliable relationship between data points while learning representations. However, we empirically show that the reason why they are successful is not only their label generation mechanisms, but also their unexplored designs. By studying two unsupervised person re-ID methods in a cross-method way, we point out a hard negative problem is handled implicitly by their designs of data augmentations and PK sampler respectively. In this paper, we find another simple solution for the problem, i.e., taking more positives during training, by which we generate pseudo-labels and update models in an iterative manner. Based on our findings, we propose a contrastive learning method without a memory back for unsupervised person re-ID. Our method works well on benchmark datasets and outperforms the state-of-the-art methods. Code will be made available.

==> backup/3_0317-1604.tex <==
\section{Empirical study}

In this section, we empirically study two contrastive learning methods for unsupervised person re-ID on Market-1501~\cite{zheng2015scalable} dataset: MMCL~\cite{wang2020unsupervised}~\footnote{MMCL can be treated as a contrastive learning method since it has a similar loss formulation with multi-labels.} and SpCL$^\dagger$~\cite{ge2020self}~\footnote{We denote the unsupervised version of SpCL as SpCL$^\dagger$.}.
Performance is evaluated by cumulative matching characteristic (CMC) curve and mean average precision (mAP)~\cite{zheng2015scalable}.
We pay attention to what might contribute to promising performance in the filed of unsupervised person re-ID.


% -----------------
\subsection{Data augmentation}

\input{floats/tab_aug_pk.tex}

In \tabref{tab:aug_pk} we study the effect of data augmentations.
Unsupervised person re-ID methods are successful using different data augmentation recipes.
However, the behaviors of data augmentations have not been studied in a cross-method way.
We denote their data augmentation modules as $\mathcal{T}_{\text{MMCL}}$ and $\mathcal{T}_{\text{SpCL$^\dagger$}}$ respectively.
Generally, $\mathcal{T}_{\text{SpCL$^\dagger$}}$ is a standard and simple person re-ID augmentation module while $\mathcal{T}_{\text{MMCL}}$ is a more sophisticated one.
Detailed augmentations are described in the supplement.

We note that performance of MMCL drops significantly if using data augmentations from SpCL$^\dagger$.
This observation is unsurprising since MMCL acts as an instance-level representation learning method (\ie, contrastive learning in a self-supervised manner) at the first several epochs, spreading instances of the same identity apart.
% TODO: better words
In this case, a simple data augmentation module such as $\mathcal{T}_{\text{SpCL$^\dagger$}}$ makes the model quickly overfit to a uniform feature distribution and lose the ability to find possible positives when it starts to mine neighbors.
In contrast, various augments slow down this process and escort the model to the neighbors-mining stage.

However, SpCL$^\dagger$ is approximate to instance-level learning at the starting, since data points are unable to be well clustered that time.
It finally archives good performance with its simple data augmentations.
We believe that SpCL$^\dagger$ reduces the negative impact of contrastive learning in unsupervised cases by an important design, \ie, PK sampler.


% -----------------
\subsection{PK sampler}

PK sampler is a common setting in the field of supervised person re-ID~\cite{hermans2017defense,luo2019bag}.
It randomly chooses $P$ identities and $K$ instances for each identity from the dataset as a batch during training.
Meanwhile, this sampling strategy is also widely used in the unsupervised cases~\cite{zeng2020hierarchical,ge2020self}.
When ground truths are unavailable, PK sampler is implemented on top of pseudo-labels.

In \tabref{tab:aug_pk} we remove the PK sampler in SpCL$^\dagger$.
Without the sampling strategy, the performance of SpCL$^\dagger$ drops a lot, similar to the behavior of MMCL when its $\mathcal{T}_{\text{MMCL}}$ is replaced.
Our explanation is that SpCL$^\dagger$ can reform data distribution and focus on the organized batches at every iteration by the PK sampler.
With that design, the model are offered more positives for each data point and escape from the force of contrastive learning, compared to that using a random sampling.


% -----------------
\subsection{Summary}

We have empirically shown a problem that models have to deal with a force which spreads positive examples apart during training without ground truths using contrastive learning.
Intuitively, this problem exists in unsupervised person re-ID scenarios even models are optimized with other losses (\eg, triplet loss).
The sophisticated data augmentations, sampling strategy may reduce the negative impact.
In summary, the model needs to be offered with more possible positive examples against that force.


% -----------------
\subsection{Hypothesis}
\label{sec:3.hypotheis}

We discuss a hypothesis on what is the core element making unsupervised person re-ID work and produce good results.
Our hypothesis is that preventing models from overfitting to an uniform feature distribution at the start of training is important.

As a proof, we increase the threshold of its self-paced clustering and get a significant gain on performance (SpCL$^\dagger$+ in \tabref{tab:aug_pk}).

In this paper, we propose another solution: introduce more positives by increasing the threshold of clustering.


==> floats/tab_epsilon.tex <==
\begin{table}
\centering
\resizebox{0.6\linewidth}{!}{
\begin{tabular}{@{}ccccc@{}}
\toprule
 & \multicolumn{2}{c}{SpCL$^\dagger$} & \multicolumn{2}{c}{TMP} \\
$\epsilon$ & mAP & Rank-1 & mAP & Rank-1 \\
\midrule
0.5 & \\
0.6 & \\
0.7 & \\
0.75 &  \\
\bottomrule
\end{tabular}
}
\caption{Effect of batch size $N$.}
\end{table}

==> floats/tab_uda.tex <==
\begin{table*}[!t]
\centering
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{3}{c}{Market-1501} & \multicolumn{3}{c}{DukeMTMC-reID} \\
method & source & mAP & Rank-1 & source & mAP & Rank-1 \\
\midrule
BUC &  & &  
38.3 & 66.2 & 27.5 & 47.4 \\
HTC \\
MMCL~\cite{wang2020unsupervised} &
128 & $\checkmark$ &
45.5 & 80.3 & 40.2 & 65.2 \\
MMCL (repro.)~\cite{wang2020unsupervised} &
128 & $\checkmark$ & 
49.9 & 81.4 & 45.6 & 66.5 \\
SpCL$^\dagger$~\cite{ge2020self} &
64 & $\checkmark$ &
73.1 & 88.1 & - & - \\
SpCL$^\dagger$~\cite{ge2020self} (repro.) &
64 & $\checkmark$ &
- & - & 63.0 & 78.6 \\
\midrule
TMP & Duke & 76.3 & 91.5  \\
\bottomrule
\end{tabular}
\caption{Comparisons on Market-1501~\cite{zheng2015scalable} and DukeMTMC-reID~\cite{ristani2016performance} under transfer learning setting.
Duke: Use DukeMTMC-reID as the source dataset.
Market: Use Market-1501 as the source dataset.
}
\label{tab:uda}
\end{table*}

